Resource Aware Person Re-identification across Multiple Resolutions

Not all people are equally easy to identify: color statistics might be enough for some cases while others might require careful reasoning about high- and low-level details. However, prevailing person re-identification(re-ID) methods use one-size-fits-all high-level embeddings from deep convolutional networks for all cases. This might limit their accuracy on difficult examples or makes them needlessly expensive for the easy ones. To remedy this, we present a new person re-ID model that combines effective embeddings built on multiple convolutional network layers, trained with deep-supervision. On traditional re-ID benchmarks, our method improves substantially over the previous state-of-the-art results on all five datasets that we evaluate on. We then propose two new formulations of the person re-ID problem under resource-constraints, and show how our model can be used to effectively trade off accuracy and computation in the presence of resource constraints. Code and pre-trained models are available at https://github.com/mileyan/DARENet.

==> anytime_budget_batch.tex <==
We now show results on person re-ID under resource-constrained scenarios described in Section~\ref{sec:resource-constrained}.
All experiments in this section are conducted on Market-1501 dataset.
%Note that this is a new problem and no previous work exists on this problem.
% has attempted to tackle the constrained re-ID.

\vspace{-1ex}
\subsubsection{Anytime person re-ID}
\vspace{-1ex}
%In the anytime person re-ID setting, re-ID system should
\label{sec:exp_anytime}

%\todo{baseline model description for the anytime settings.}
\paragraph{Baselines:} We compare our \nameshort{} model against sequentially evaluated three ResNets (SE-ResNets)~\cite{he2016deep}: a ResNet18, a ResNet34 and a ResNet50 where we used the largest net that fits in the budget.
All three ResNet models are trained separately using the same triplet loss as in \cite{hermans2017defense}.
At test time, the networks are evaluated sequentially in ascending order of size, and are forced to output the most recent re-ID result after surpassing the budget limit.

\paragraph{Anytime re-ID results:} Figure~\ref{fig:anytime} summarizes the results of the anytime setting. The computational cost is reported with respect to the cumulative number of  multiplications and additions 
(Mul-Add). We confirm that the actual running timing is consistent with the Mul-Add.
Note that we cannot perform re-ranking~\cite{zhong2017re} in this setting since we cannot assume all queries are available at once.
So we report the results from model ``\nameshort{}+RE'' in Table ~\ref{main_results}.

Except for a narrow range of budgets, our \nameshort{} model outperforms the SE-ResNets significantly.
In particular, our model is able to achieve a high accuracy very quickly, achieving $3 \sim 5$ points higher performance for budgets higher than $2.5 \times 10^9$ Mul-Adds.
This is because unlike the SE-ResNets, ours is a single model that \emph{shares} computation between the quick-and-dirty and the slow-and-accurate predictions.
%Our model is especially able to provide state-of-the-art Especially on budget ranging from $2.5 \times 10^9$ to $5.5 \times 10^9$, our \nameshort{} model achieves $3\sim5\%$ higher CMC rank 1 accuracy.



%\subsubsection{Budgeted batch person re-ID}
%\label{sec:exp_budgeted_batch}
%\paragraph{Confidence - CMC rank 1 accuracy relationship} We show the relationship between the nominal confidence and CMC rank 1 accuracy in Figure \todo{ADD the conf-acc figure}.
%\yy{should I add 1 or all four figure on this topic? since we have four stages.}

%\paragraph{Models}

%\paragraph{Budgeted batch re-ID results} Since no other models have considered such setting, we estimate the computation resource consumption at inference of several state-of-the-art models and plot the corresponding points.
%We also show the performance of the individual embeddings from each stage.
%The distance-based exit strategy outperforms most other models significantly, as seen in Figure ~\ref{fig:budget}.
%Importantly, it is able to correctly trade-off heavy computation on the hard examples with quick prediction on the easy examples, achieving higher accuracy with lower cost than the individual embeddings.
%The LP problem of random exit strategy is solved under $Q^i$ as overall CMC rank 1 at stage $i$, and the confidence-based exit strategy is conducted on choosing $\alpha = \beta = 1$.

%It can be seen that even though we do not incorporate any special design on $\{p_i\}$ under budget $B$, in terms of budget-accuracy trade-off, the distance-based exit strategy outperforms surpassed most other models significantly.

\begin{figure}[!tb]
	\centering
	\includegraphics[width=\linewidth]{./figures/anytime_and_budgeted_batch/anytime2.pdf}
	\caption{CMC rank 1 accuracy under \textit{anytime re-ID} setting as a function of the  computational budget on the Market-1501 dataset.}
\vspace{-2ex}
	\label{fig:anytime}
\end{figure}


%\begin{figure}[!tb]
%	\centering
%	\includegraphics[width=0.8\linewidth]{./figures/anytime_and_budgeted_batch/budget_batch_reranking}
%	\caption{CMC rank 1 accuracy under \textit{budgeted batch re-ID} setting as a function of computational budget on Market 1501 dataset. Higher is better. Here we follow the same naming in Table.~\ref{main_results}, and use ``\nameshort{}+RE dist-exit'' for the model that adopts the distance-based early exit strategy, ``\nameshort{}+RE'' for model only using one stage output (thus has 4 points in the figure).
%	}
%	\label{fig:budget}
%\end{figure}


==> anytime_stream.tex <==
\vspace{-1ex}
\subsubsection{Budgeted stream person re-ID}
\vspace{-1ex}
\label{sec:stream}

\begin{figure}[!tb]
	\centering
	\includegraphics[width=\linewidth]{./figures/anytime_and_budgeted_batch/budgeted_stream_detail.pdf}
	\caption{Results on the Market data set under the budgeted streaming setting. The graph shows the CMC Rank 1 accuracy as a function of the average budget in terms of Mul-Add.  }
\vspace{-2ex}
	\label{fig:stream}
\end{figure}
%\paragraph{Budgeted stream re-ID results}
Figure~\ref{fig:stream} shows the results in the budgeted streaming setting. We compare three variants of \nameshort{} with four stages.  Each variant uses a different method to exit queries early. In the \emph{random} setting, we interpolate between the individual stages (indicated as blue points). The straight lines between the blue dots are obtained by randomly deciding to exit queries at either one of the two corresponding stages, which yields a smooth interpolation between the budgets of the two stages. In the \emph{distance} variant, the top $q_s$ fraction with the shortest distance to their nearest gallery neighbor is exited at each stage. In the \emph{margin} variant inputs are exited based on their margin of certainty between the nearest neighbor and the second nearest neighbor of a different class. This latter version assumes the knowledge of class labels of gallery data points.
%We compute the Pareto-optimal thresholds on a validation set held out from the training set: $20\%$ of the examples are used for validation.
We observe that our choice of thresholds are able to route queries effectively, allowing us to achieve higher accuracy at lower cost comparing to other prior state-of-the-art models (which are only single points without the ability to trade-off accuracy for computational cost). In the presence of training labels the \emph{margin} selection method is clearly preferred over the \emph{distance} based method. Both methods clearly outperform random interpolation.
%Note that the thresholds tuned on the validation set may no longer be Pareto-optimal on the test set, nevertheless, Figure~\ref{fig:stream} shows that they still work quite well.

%We do it by training a new run and splitting the training set into 2 parts, $80\%$ for training network, and $20\%$ act as validation set to search for threshold strategies. Then we take this threshold strategy set, apply on the model trained by the whole training set and test it on test set. Since we search the threshold strategies on validation set, and test these strategies without modification on test set, so it's possible that the \emph{Performance--Budget} curve on test set not being convex.


%\bh{Use for supplementary}
%\paragraph{Evaluation of Threshold Strategies}
%We evaluate the threshold strategies by checking its exit probability on each stage on test set. The searched strategies shows that the best exit policies are not to focus on the balance of every exits, but rather ignore some and make full use of others. Table ~\ref{anytime_result} shows the exit probability of our strategy set on test set.
%\begin{table*}[]
%\centering
%\begin{tabular}{lcccccccccc}
%\hline
%\multicolumn{6}{c}{Threshold Strategies exit probability} \\
% \hline
% Strategy id &Budget(Mflops) & Exit1($\%$) & Exit2 ($\%$) & Exit3($\%$) & Exit4($\%$) \\
% 1& 555 & 95.4$\%$ & 4.4$\%$ & 0 & $0.2\%$ \\
%  2& 605 & 90.4$\%$ & 7.7$\%$ & 1.6$\%$ & $0.2\%$ \\
%3& 644 & 86.5$\%$ & 10.8$\%$ & 1.4$\%$ & $1.2\%$ \\
%4& 688 & 76.7$\%$ & 22.5$\%$ & 0.7$\%$ & $0.2\%$ \\
%5& 724 & 76.7$\%$ & 18.9$\%$ & 4.0$\%$ & $0.4\%$ \\
%6& 749 & 73.7$\%$ & 21.3$\%$ & 4.5$\%$ & $0.5\%$ \\
%7& 853 & 69.4$\%$ & 18.3$\%$ & 10.6$\%$ & $1.6\%$ \\
%8& 994 & 58.2$\%$ & 23.4$\%$ & 16.2$\%$ & $2.3\%$ \\
%9& 1008 & 55.0$\%$ & 27.5$\%$ & 15.0$\%$ & $0.3\%$ \\
%10& 1107 & 50.0$\%$ & 28.8$\%$ & 12.8$\%$ & $8.4\%$ \\
%11& 1346 & 44.6$\%$ & 25.3$\%$ & 0 & $30.1\%$ \\
%12& 1699 & 32.0$\%$ & 20.0$\%$ & 0 & $48.0\%$ \\
%13& 1964 & 17.0$\%$ & 0 & 67.5$\%$ & $15.6\%$ \\
%\hline
%\end{tabular}
%\caption{Anytime stream strategies}
%\label{anytime_result}
%\end{table*}




==> notations.tex <==
training dataset: X
training example: x^i
training Labels:Y
Batch_i: S_i
Label of Batch_i: H_i
Query set: \mathcal{Q}
Query example: q^i
Gallery set: \mathcal{G}
Gallery example:g^i
Budget: B
number of examples in the Query set: M
parameter of neural network: \theta
neural network function: f_{\theta}
output of neural network function: f(q^i)/f(g^i)/f(x^i)
anchor image: x_a^i
positive example: x_p^i
negative example: x_n^i
margin: \alpha
triplet loss: L
batch hard triplet loss:L_{BH}
In a batch, we sample C classes, each class K images
soft-margin: s
soft-margin parameter: \beta
feature of batch i after block j: {F_i^j}




==> problem_setup.tex <==

%\yy{Should we emphasize the practical significance of such setting here?}
%\lw{can fist wirte it and then we simplify it}
% Such setting is also of highly practical significance.

%
%In the supervised person re-identification problem, we are given a set of images $X$ which  persons and their labeled identities $I$. Our goal is to learn a model from the labeled dataset to identify whether two images which might have not been seen in the training set are of the same person or not.
%
%During testing, we are given a set of images $X_{g}$ as gallery set we have collected in advance. We observe a set of probe images $X_{p}$ and our goal is to retrieve images of the same person in the gallery set as images in the probe set.
%

% Problem statement by Xu
% A person re-identification problem is such a problem that, given some images as "probe" image,  and a "gallery" which contains many sets of images of different people from another camera. Our goal is to figure out which person in the "gallery" set does the given images belong to.

% A typical setting of this problem is that, the training sets have images of some people from different cameras, while the test set contains images of people other than those in the train set. So we cannot treat it as a simple classification problem since the people in our test dataset are different from those in the train set.

% To deal with such problem, instead of directly learning labels for each image, we learn an encoder, which turns the input image to a feature vector. The encoder shall fulfill the following properties:1 , images from different cameras of the same person shall be encoded close. 2, images of different people shall be encoded far away in Euclidean distance. With such an encoder, given a "probe" image, we can do re-identification by choosing the feature vector in the gallery which is closest to the "probe" vector.

%\subsubsection{Anytime Prediction}


